Results of the Photometric LSST Astronomical Time-series Classification Challenge (PLAsTiCC)

Next-generation surveys like the Legacy Survey of Space and Time (LSST) on the Vera C. Rubin Observatory will generate orders of magnitude more discoveries of transients and variable stars than previous surveys. To prepare for this data deluge, we developed the Photometric LSST Astronomical Time-series Classification Challenge (PLAsTiCC), a competition which aimed to catalyze the development of robust classifiers under LSST-like conditions of a non-representative training set for a large photometric test set of imbalanced classes. Over 1,000 teams participated in PLAsTiCC, which was hosted in the Kaggle data science competition platform between Sep 28, 2018 and Dec 17, 2018, ultimately identifying three winners in February 2019. Participants produced classifiers employing a diverse set of machine learning techniques including hybrid combinations and ensemble averages of a range of approaches, among them boosted decision trees, neural networks, and multi-layer perceptrons. The strong performance of the top three classifiers on Type Ia supernovae and kilonovae represent a major improvement over the current state-of-the-art within astronomy. This paper summarizes the most promising methods and evaluates their results in detail, highlighting future directions both for classifier development and simulation needs for a next generation PLAsTiCC data set.

==> Makefile <==
# To make the document with the default settings:
# > make
#
# To make with a specific format:
# > make <format>
#
# To tar up a flat version of a specific format:
# > make <format> tar
#
# Alex Drlica-Wagner: https://github.com/LSSTDESC/start_paper/issues/new?body=@kadrlica

# Primary file names - avoid cookiecutter variables, to enable `make
# upgrade` to cleanly over-write this Makefile...
main ?= main
#default=$(shell cat .metadata.json | grep 'default_format' | cut -d'"' -f4)
outname ?= $(notdir $(shell pwd))

#ifeq ($(default), {{ cookiecutter.default_format }})
style ?= lsstdescnote
#else
# style=${default}
#endif

# 'note' shall be an alias for 'lsstdescnote'
ifeq ($(style),note)
style = lsstdescnote
endif
# mkauthlist doesn't recognize lsstdescnote as a style, so tell it to do something generic
ifeq ($(style),lsstdescnote)
mastyle = tex
else
mastyle = $(style)
endif

DESCTEX := desc-tex
DESCTEXORIGIN := git@github.com:LSSTDESC/desc-tex.git
LSSTTEX := lsst-texmf
LSSTTEXORIGIN := git@github.com:lsst/lsst-texmf.git

localpip ?= F
PIPOPTS = --upgrade-strategy only-if-needed
ifeq ($(localpip),T)
MKAUTHBIN := bin/mkauthlist
MKAUTH := PYTHONPATH=$$(ls -d lib/python*/site-packages 2>/dev/null | head -n1):$$PYTHONPATH $(MKAUTHBIN)
PIPOPTS += --install-option="--prefix=$(PWD)"
GETMKAUTH := [ -e $(MKAUTHBIN) ] || pip install $(PIPOPTS) mkauthlist
else
MKAUTHBIN :=
MKAUTH := mkauthlist
GETMKAUTH := pip list 2>/dev/null | grep -q mkauthlist || pip install $(PIPOPTS) mkauthlist
endif

# LATEX environment variables
export TEXINPUTS:=./$(DESCTEX)/styles/:./tables/:
export BSTINPUTS:=./$(DESCTEX)/bst/:
export BIBINPUTS:=./$(DESCTEX)/bib/:./$(LSSTTEX)/texmf/bibtex/bib/:

# LaTeX journal class switcher flags
# apj=\def\flag{apj}
# apjl=\def
# mnras=\def\flag{mnras}

# Submission flags (these need some thought)
# arxiv=\def\flag{emulateapj}
# submit=${aastex}
draft=\def\linenums{}# {\linenumbers}

# Files to copy when making tarball
tardir := tmp
figdir ?= ./figures
figures ?= $(figdir)/*.{png,jpg,pdf}
tabdir ?= ./tables
tables ?= $(tabdir)/*.tex
styles ?= ./$(DESCTEX)/styles/*.{sty,cls}
bibs ?= ./$(DESCTEX)/bib/*.bst
source = $(main).{tex,bbl,bib} $(DESCTEX)/bib/lsstdesc.bib $(DESCTEX)/ack/*.tex authors.tex contributions.tex $(LSSTTEX)/texmf/bibtex/bib/lsst.bib $(LSSTTEX)/texmf/bibtex/bib/lsst-dm.bib

tarfiles = $(figures) $(tables) $(styles) $(bibs) $(source)

# prefix for difference files
DIFPRE ?= diff_
# git repo branch to compare changes against
BASEBRANCH ?= master
# git repo branch we are compiling
THISBRANCH := $(shell git branch --no-color 2> /dev/null | sed -e '/^[^*]/d' -e 's/* \(.*\)/ \1/' | tr -d ' ')
# temp file for the version to compare against
DRAFT = $(main).$(BASEBRANCH)
# base for difference files to generate
DIFF = $(DIFPRE)$(THISBRANCH)--$(BASEBRANCH)


maketargets := all authlist clean copy diff help $(main) update tar templates tidy touch
.PHONY: $(maketargets)

styleopts := aastex61 apj apjl emulateapj lsstdescnote mnras note prd prl tex
help:
	@echo "Usage: make [style=lsstdescnote] [localpip=F] <target(s)>\n Possible targets: $(maketargets) <style> $(DESCTEX) $(LSSTTEX)\n  all: equivalent to 'make $(main) copy'\n  authlist: use mkauthlist to generate latex author/affiliation listing\n  clean: remove latex temporary files AND compiled outputs\n  copy: copy $(main).pdf to $(outname).pdf\n  diff: if we're in a git repo, use latexdiff to compare the current $(main).tex vs the $(BASEBRANCH) branch, and attempt to compile to $(DIFF).pdf\n  help: what you're looking at\n  $(main): compile $(main).tex\n  update: update desc-tex, mkauthlist, and templates repo\n  tar: tar up latex source files to $(outname).tar.gz\n  templates: download latest templates to templates/\n  tidy: delete latex temporary files\n  touch: touch $(main).tex to force a recompile\n  <style>: equivalent to 'make style=<style> $(main) copy tar' (see style option)\n  $(DESCTEX): download $(DESCTEX), which provides the DESC header logo and latex helper files (done automatically on first latex compilation)\n  $(LSSTTEX): download $(LSSTTEX), providing (among other things) LSST project bib files (not done automatically)\n Options for style: $(styleopts) (Anything else results in generic latex)\n Options for localpip: T or F. Set to T to install mkauthlist in this directory rather than systemwide"


# Interpret `make` with no target as `make tex` (a latex Note).
# At present, if the default_format is anything other than
# [apj|apjl|mnras|prd|prl|emulateapj], a latex Note is made.
# In future, we could think of using `make` to eg run the ipynb
# notebook and make PDF from the output, but this has not been
# implemented yet.
$(main): export flag = \def\flag{${style}}
envflag = \\def\\flag{${style}}
all: $(main) copy

copy:
	cp ${main}.pdf ${outname}.pdf

touch:
	touch ${main}.tex

# if we are in a git repo, add as a submodule; otherwise clone
$(DESCTEX):
	if [ -d .git ]; then git submodule add $(DESCTEXORIGIN); else git clone $(DESCTEXORIGIN); fi
$(LSSTTEX):
	if [ -d .git ]; then git submodule add $(LSSTTEXORIGIN); else git clone $(LSSTTEXORIGIN); fi

#http://journals.aas.org/authors/aastex/linux.html
#change the compiler call to allow a "." file
# {% raw %}
$(main) : $(DESCTEX) authlist
	STYLEFLAG=$(envflag) latexmk $(main)
#	latexmk -g -pdf  \
	-pdflatex='openout_any=a pdflatex %O -interaction=nonstopmode "${flag}\input{%S}"'  \
	${main}
# {% endraw %}

diff: $(DIFF).pdf
$(DIFF).pdf: $(DIFF).tex
	STYLEFLAG=$(envflag) latexmk $<
$(DIFF).tex: $(DRAFT).tex $(main).tex
	latexdiff --exclude-textcmd="multicolumn" $^ > $@
# this ensures that the version to latexdiff against is always updated
.PHONY: $(DRAFT).tex
$(DRAFT).tex:
	if git show $(BASEBRANCH):$(main).tex > $@; then true; else echo "\n\n'make diff' is intended to be used inside a git repository\n"; false; fi



tar : $(main)
	mkdir -p ${tardir}
	cp ${tarfiles} ${tardir} | true
	cp ${outname}.pdf ${tardir}/${outname}.pdf
	cd ${tardir} && tar -czf ../${outname}.tar.gz . && cd ..
	rm -rf ${tardir}

authlist: authors.tex
authors.tex : authors.csv
	$(GETMKAUTH)
	$(MKAUTH) -j ${mastyle} -f -c "the LSST Dark Energy Science Collaboration \\ and \\ the LSST Transients and Variable Stars Science Collaboration" \
		--cntrb contributions.tex authors.csv authors.tex
#	pip install --upgrade mkauthlist


# http://stackoverflow.com/q/8028314/
.PHONY: $(styleopts)
$(styleopts): export style = $(@)
$(styleopts): export flag = \def\flag{$(@)}
$(styleopts):
	$(MAKE) -e $(main)
	$(MAKE) -e copy
	$(MAKE) -e tar
# NB. the 'tex' target doesn't actually do anything in docswitch - make
# with no target compiles PDF out of main.tex using lsstdescnote.cls
# (which is to say, by default we assume you are writing an LSST
# DESC Note in latex format).

tidy:
	rm -f *.log *.aux *.out *.dvi *.synctex.gz *.fdb_latexmk *.fls
	rm -f *.bbl *.blg *Notes.bib ${main}.pdf

clean: tidy
	rm -f ${outname}.pdf ${outname}.tar.gz

# Update the tex styles etc:

baseurl=https://raw.githubusercontent.com/LSSTDESC/start_paper/deploy

# UPDATES=\
# texmf/bib/apj.bst \
# texmf/bib/mnras.bst \
# texmf/styles/aas_macros.sty \
# texmf/styles/aastex.cls \
# texmf/styles/aastex61.cls \
# texmf/styles/aps_macros.sty \
# texmf/styles/docswitch.sty \
# texmf/styles/emulateapj.cls \
# texmf/styles/mnras.cls \
# texmf/styles/lsstdescnote.cls \
# texmf/styles/lsstdesc_macros.sty \
# texmf/logos/desc-logo-small.png \
# texmf/logos/desc-logo.png \
# texmf/logos/header.png \
# lsstdesc.bib \
# .travis.yml \
# figures/example.png

# .PHONY: $(UPDATES)
# $(UPDATES):
# 	curl -s -S -o $(@) ${baseurl}/$(@)
# 	@echo " "

update: templates
	@echo Updating desc-tex
	cd $(DESCTEX) && git pull
	@echo
	@echo Updating mkauthlist
	pip install --upgrade $(PIPOPTS) mkauthlist
#@echo "\nOver-writing LaTeX style files with the latest versions: \n"
#@mkdir -p .logos figures texmf/styles texmf/bib
#$(MAKE) $(UPDATES)

# Get fresh copies of the templates etc, for reference:
# It is a bad idea to make these phony targets

TEMPLATES:=\
authors.csv \
main.ipynb \
main.md \
main.rst \
main.tex \
main.bib \
Makefile
#.metadata.json \
#.travis.yml
#figures/example.png
# #acknowledgments.tex \

ALLTEMPLATES := $(TEMPLATES) header.png

# .PHONY: $(TEMPLATES)
# $(TEMPLATES):
# 	curl -s -S -o templates/$(@) ${baseurl}/$(@)
# 	@echo " "

gettemplates := $(foreach t,$(TEMPLATES),curl -s -S -o templates/$(t) ${baseurl}/$(t); )

# NB: fetching header.png will fail as long as desc-tex is private
templates:
	@echo "\nDownloading the latest versions of the template files, for reference: \n"
	@mkdir -p templates
	$(gettemplates)
	curl -f -s -S -o templates/header.png https://raw.githubusercontent.com/LSSTDESC/desc-tex/master/logos/header.png || true
	@echo
	@echo templates/ listing:
	@ls -a templates/*
	@for f in $(ALLTEMPLATES); do diff -q $$f templates/$$f; true; done
#$(MAKE) $(TEMPLATES)
#	$(MAKE) new

# Get a template copy of the latest Makefile, for reference:
# new:
# 	@echo "\nDownloading the latest version of the Makefile, for reference: \n"
# 	@mkdir -p templates
# 	curl -s -S -o templates/Makefile ${baseurl}/Makefile
# 	@echo " "

# Over-write this Makefile with the latest version:
# Why would we include this when a safe option already exists?
# upgrade:
# 	@echo "\nDownloading the latest version of the Makefile: \n"
# 	curl -s -S -o Makefile ${baseurl}/Makefile
# 	@echo "\nUpgrading version of mkauthlist: \n"
# 	pip install mkauthlist --upgrade --no-deps
# 	@echo "\nNow get the latest styles and templates with\n\n    make update\n    make templates\n"


==> authors.tex <==
% Author list file generated with: mkauthlist 1.2.4 
% mkauthlist -j apj -f -c LSST Dark Energy Science Collaboration --cntrb contributions.tex authors.csv authors.tex 

\author{R.~Hlo\v{z}ek}
\affiliation{Department of Astronomy and Astrophysics, University of Toronto, 50 St. George St., Toronto, ON M5S 3H4, Canada}
\affiliation{Dunlap Institute for Astronomy and Astrophysics, University of Toronto, 50 St. George St., Toronto, ON M5S 3H4, Canada}
\author{K.~A.~Ponder}
\affiliation{Berkeley Center for Cosmological Physics, Campbell Hall 341, University of California Berkeley, Berkeley, CA 94720, USA}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720, USA}
\affiliation{SLAC National Accelerator Laboratory, 2575 Sand Hill Rd, Menlo Park, CA 94025, USA}
\author{A.I.~Malz}
\affiliation{Ruhr University Bochum, German Centre of Cosmological Lensing, Universitaetsstra{\ss}e 150, 44801 Bochum, Germany}
\author{M.~Dai}
\affiliation{Department of Physics and Astronomy, Johns Hopkins University, Baltimore, MD 21218, USA}
\affiliation{Rutgers, the State University of New Jersey, 136 Frelinghuysen Road, Piscataway, NJ 08854 USA}
\author{G.~Narayan}
\affiliation{Space Telescope Science Institute, 3700 San Martin Dr, Baltimore, MD 21218, USA}
\author{E.E.O.~Ishida}
\affiliation{Universit\'e Clermont Auvergne, CNRS/IN2P3, LPC, F-63000 Clermont-Ferrand, France}
\author{T.~Allam Jr}
\affiliation{Mullard Space Science Laboratory, Department of Space and Climate Physics, University College London, Holmbury Hill Rd, Dorking RH5 6NT, UK}
\author{A.~Bahmanyar}
\affiliation{Dunlap Institute for Astronomy and Astrophysics, University of Toronto, 50 St. George St., Toronto, ON M5S 3H4, Canada}
\author{R.~Biswas}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, AlbaNova, Stockholm, SE-106 91, Sweden}
\author{L.~Galbany}
\affiliation{Departamento de F\'isica Te\'orica y del Cosmos, Universidad de Granada, E-18071 Granada, Spain}
\author{S.W.~Jha}
\affiliation{Rutgers, the State University of New Jersey, 136 Frelinghuysen Road, Piscataway, NJ 08854 USA}
\author{D.~O.~Jones}
\affiliation{NASA Einstein Fellow, University of Santa Cruz, 1156 High St, Santa Cruz, CA 95064, USA}
\author{R.~Kessler}
\affiliation{KICP, 5640 S Ellis Ave, Chicago, IL 60637}
\author{M.~Lochner}
 \affiliation{Department of Physics and Astronomy, University of the Western Cape, Bellville, Cape Town, 7535, South Africa}
 \affiliation{South African Radio Astronomy Observatory (SARAO), 2 Fir Street, Observatory, Cape Town, 7925, South Africa}
\affiliation{African Institute for Mathematical Sciences, 6 Melrose Road, Muizenberg, 7945, South Africa}
\author{A.A.~Mahabal}
\affiliation{Division of Physics, Mathematics, and Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation{Center for Data Driven Discovery, California Institute of Technology, Pasadena, CA 91125, USA}
\author{K.S.~Mandel}
\affiliation{Institute of Astronomy and Kavli Institute for Cosmology, Madingley Road, Cambridge, CB3 0HA, UK}
\affiliation{Statistical Laboratory, DPMMS, University of Cambridge, Wilberforce Road, Cambridge, CB3 0WB, UK}
\author{J.R.~Mart\'inez-Galarza}
\affiliation{Center for Astrophysics | Harvard \& Smithsonian, 60 Garden Street, Mail Stop 66 Cambridge, MA 02138}
\author{J.D.~McEwen}
\affiliation{Mullard Space Science Laboratory, Department of Space and Climate Physics, University College London, Holmbury Hill Rd, Dorking RH5 6NT, UK}
\author{D.~Muthukrishna}
\affiliation{Institute of Astronomy and Kavli Institute for Cosmology, Madingley Road, Cambridge, CB3 0HA, UK}
\author{H.V.~Peiris}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, AlbaNova, Stockholm, SE-106 91, Sweden}
\affiliation{Department of Physics and Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\author{C.M.~Peters}
\affiliation{Dunlap Institute for Astronomy and Astrophysics, University of Toronto, 50 St. George St., Toronto, ON M5S 3H4, Canada}
\author{C.N.~Setzer}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, AlbaNova, Stockholm, SE-106 91, Sweden}

\collaboration{LSST Dark Energy Science Collaboration, LSST Transient and Variable Stars Collaboration}


==> latexmkrc <==
# Choose which style to pass to docswitch
# NB: Default value here is always used by Overleaf
$theflag = $ENV{'STYLEFLAG'} || '\def\flag{lsstdescnote}';

# Set environment variables to search for tex inputs
# http://tex.stackexchange.com/a/50847/121099
$ENV{'TEXINPUTS'}='./desc-tex/:./tables/:' . $ENV{'TEXINPUTS'};
$ENV{'BSTINPUTS'}='./desc-tex/bib/:' . $ENV{'BSTINPUTS'};

# Set control tools
$go_mode = 1;
$pdf_mode = 1;
# You can change the \flag value here...
$pdflatex = 'openout_any=a pdflatex %O -interaction=nonstopmode "' . $theflag . '\input{%S}"'

